Improving Online Source-free Domain Adaptation for Object Detection by Unsupervised Data Acquisition

Effective object detection in autonomous vehicles is challenged by deployment in diverse and unfamiliar environments. Online Source-Free Domain Adaptation (O-SFDA) offers model adaptation using a stream of unlabeled data from a target domain in an online manner. However, not all captured frames contain information beneficial for adaptation, especially in the presence of redundant data and class imbalance issues. This paper introduces a novel approach to enhance O-SFDA for adaptive object detection through unsupervised data acquisition. Our methodology prioritizes the most informative unlabeled frames for inclusion in the online training process. Empirical evaluation on a real-world dataset reveals that our method outperforms existing state-of-the-art O-SFDA techniques, demonstrating the viability of unsupervised data acquisition for improving the adaptive object detector.

==> sections/table_seq_shift2city_267.tex <==
\begin{table}[t]
\centering
\caption{Shift to Sequential Cityscapes on Frankfurt Validation Set }
\label{tab:Shift to Sequential Cityscapes}
%\scalebox{0.8}{
\resizebox{1\linewidth}{!}{
\begin{tabular}{
l|cccc|c}
\toprule
\textbf{Method} &  Person & Car & Mcycle & Bike & \textbf{mAP Frankfurt} \\
\midrule
Source-Only& 16.1  & 17.1  & 4.5  & 6.1 & 10.9  \\
\midrule
Tent$^{\dagger}$~\cite{wang2021tent}&16.5±0.3	&18.0±0.0&	8.1±2.2&	6.5±2.4	&12.3±1.1\\
MemCLR~\cite{vs2023towards}   & 22.1±0.5  & 25.3±0.5  & 9.9±1.2  & 8.7±0.8 & 16.5±0.4 \\

\cellcolor{c1}\textbf{Ours} & \cellcolor{c1}\textbf{30.2±0.8}  & \cellcolor{c1}\textbf{39.5±0.9}&\cellcolor{c1}\textbf{21.9±3.4}& \cellcolor{c1}\textbf{11.7±1.2}  & \cellcolor{c1}\textbf{25.8±0.8} \\
\bottomrule
\end{tabular}
}
\end{table}



==> sections/table_seq_sim2city.tex <==
\begin{table}[t]
\centering
\caption{Sim10k to Sequential Cityscapes (Car only)}
\label{tab:sim10k to sequential cityscapes(car only)}
\setlength{\tabcolsep}{10mm}{
\begin{tabular}{lc}
\toprule
   \textbf{Method}       & Car  \\ 
\midrule
 Source-Only                                                                     & 31.9 \\ 
\midrule
Tent$^{\dagger}$~\cite{wang2021tent}&33.1±0.3\\
 MemCLR~\cite{vs2023towards}                                                                            & 37.0±0.2\\
\cellcolor{c1}\cellcolor{c1}\textbf{Ours}                                 & \cellcolor{c1}\cellcolor{c1}\textbf{46.0±0.2}      \\
\bottomrule
\end{tabular}}
\end{table}


